A denotational semantics for PROMELA addressing arbitrary jumps

PROMELA (Process Meta Language) is a high-level specification language designed for modeling interactions in distributed systems. PROMELA is used as the input language for the model checker SPIN (Simple Promela INterpreter). The main characteristics of PROMELA are non-determinism, process communication through synchronous as well as asynchronous channels, and the possibility to dynamically create instances of processes. In this paper, we introduce a bottom-up, fixpoint semantics that aims to model the behavior of PROMELA programs. This work is the first step towards a more ambitious goal where analysis and verification techniques based on abstract interpretation would be defined on top of such semantics.

==> wgmacros-FLP.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                         %
%   Staff only for FLPs   %
%                         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\@ifpackageloaded{MnSymbol}{}{\PackageWarning{WGmacros}%
{Please load `MnSymbol' package explicitely in preamble}
\RequirePackage{MnSymbol}}
\makeatother
% \RequirePackage{listings}

\input{wgmacros-support}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                             %
%   Subject Specific macros   %
%                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%% Weak Evolving Result Sets
\newcommand*{\WERSabsSym}{\nu}
\newcommand*{\WERS}[1][\zseq{x}]{\mathbb{WERS}_{#1}}
\newcommand*{\WERSinterps}{\Ainterps[{\WERS[]}]}
\newcommand*{\WERSinterp}{\I[\WERSabsSym]}
\monobioperator{\WERSglb}{\curlywedge}{\bigcurlywedge} %% g.l.b. on set of answer evolution trees
\monobioperator{\WERSlub}{\curlyvee}{\bigcurlyvee} %% l.u.b. on set of answer evolution trees
\newcommand*{\WERSgeq}{\succeq} %% \leqAET^{-1}
\newcommand*{\WERSleq}{\preccurlyeq} %% pre-order on answer evolution trees
\newcommand*{\WERSnleq}{\npreccurlyeq} %% pre-order on answer evolution trees

\newcommand*{\WERSF}{\F[\WERSabsSym]}
\newcommand*{\WERSTp}{\Tp[\WERSabsSym]}
\newcommand*{\WERSabs}[1][V]{\parensmathoper{\WERSabsSym_{#1}}}%\mars
\makeparensmathoper{\WERSconc}{\WERSabsSym^{\gamma}}%\mars
\newcommand*{\WERSeval}[4][V]{\mathoper{\evalSym^{\WERSabsSym}_{#1}}\ifempty{#3}{}{\BBrackets[{#4}]{\termres{#3}{#2}}}}
\newcommand*{\WERSspecRel}[4][V]{\WERSspec[#1]{#2}{#3} \vdash #4}
\newcommand*{\WERSspec}[3][V]{#2 [#3]_{#1}}
\newcommand*{\WERSzap}[2]{\parensmathoper{zap_{#1}}}%_{#2}

\newcommand*{\WERSroot}[2]{#1 \centerdot #2}%\,\sharp\,\ldotp\vdots\diamond\vdash\ssearrow
\newcommand*{\WERSseg}[3]{\WERSroot{#1}\ifempty{#2}{\emptyset}{#2}\mbox{--}\ifempty{#3}{??}{#3}}
% \newcommand*{\WERSseg}[3]{\WERSgenseg{#1}{\{#2\}}{#3}}



% \newcommand*{\ERTgenericforest}{\mathcal{F}}
\newcommand*{\eleq}[1][\Fbox{V}]{\twoheadrightarrow_{#1}}% \precapprox}
\makeparensmathoper{\shell}{\tau} %% the shell of a term

%% Definitional Trees
\makeparensmathoper{\pat}{pat}
\makeparensmathoper{\ruleNode}{rule}
\makeparensmathoper{\branchNode}{branch}
\makeparensmathoper{\orNode}{or}

\newcommand*{\CurryEval}[6][]{\syntaxoper{Eval}{\extraArgSc{#2}{#1}}{} \xRightarrow[{#5}]{\extraArg{#3}{#4}} #6}

\newcommand*{\stricteq}{\mathbin{\mlst{=:=}}}
\newcommand*{\paralland}{\mathbin{\mlst{&}}}
\newcommand*{\seqand}{\mathbin{\mlst{&>}}}
\newcommand*{\success}{\mlst{success}}

%% TERM GRAPHS MACROS
\newcommand*{\Roots}[1]{\mathcal{R}\mathclose{oot}_{#1}} %% root node
\newcommand*{\Nds}[1]{\mathcal{N}_{#1}} %% graph nodes
\newcommand*{\Lbl}[1][\Fbox{g}]{\parensmathoper{\mathcal{L}_{#1}}} %% label map
\newcommand*{\Suc}[1][\Fbox{g}]{\parensmathoper{\mathcal{S}_{#1}}} %% successor map
\newcommand*{\reach}[1]{\rightarrowtriangle_{#1}} %% reachability relation over positions of a term
\newcommand*{\nreach}[1]{\nrightarrowtriangle_{#1}} %% reachability relation over positions of a term

%% Staff relative to (CRWL) term bottom

\newcommand*{\botSym}{\bot}

\newcommand*{\botCsyms}{\Csyms_{\botSym}} %% constructor symbols
\newcommand*{\botSyms}{\Fsyms_{\botSym}} %%  symbols \cup black box

\newcommand*{\botvar}[1][]{{\varrho_{#1}}}

\newcommand*{\botVsyms}{\Vsyms_{\botvar}}
\newcommand*{\botTerms}{\SigTerms{\Csyms}{\Vsyms \cup \botVsyms}}%[1][]\ifempty{#1}{}{\Fbox{#1}}
\newcommand*{\botSubsts}{\botvar\Substs}


% \newcommand*{\cApprox}[1]{\tau_{\Cbox}(#1)}


\newcommand*{\strictvareq}{\mathrel{\doteq}}

% COMPATIBILITY

\backcompatibility{\botVsym}{\botVsyms}
\backcompatibility{\BoxCsym}{\botCsyms}
\backcompatibility{\BoxSym}{\botSyms}
\backcompatibility{\Cbox}{\botSyms}
\backcompatibility{\botSubst}{\botSubsts}
\newcommand*{\pansw}[2]{\Fbox{$#1 \cdot #2$}}%\talloblong\mathrel{}

% now load general staff

\input{wgmacros-general}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               %
%   overrides of general defs   %
%                               %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand*{\proglang}{\textsf{Curry}}
\renewcommand*{\paradigm}[1][]{#1\textsf{FLP}}


==> wgmacros-absint.tex <==
\makeatletter
\ifx\@wgmacros@absint\@relax\else\makeatother\endinput\fi
\gdef\@wgmacros@absint{\relax}
\typeout{********* LOADING wgmacros-absint}
\makeatother

\input{wgmacros-support}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%                        %
%   DOMAINS and orders   %
%                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%

% Generic Concrete Domain (for preliminaries)

\newcommand*{\CC}{\mathbb{C}}
\newcommand*{\CCleq}{\sqsubseteq} %% order on Concrete Domain
\newcommand*{\CCnleq}{\nsqsubseteq} %% negated order on Concrete Domain
\newcommand*{\CClt}{\sqsubset}
\newcommand*{\CCgeq}{\sqsupseteq} %% opposite order on Concrete Domain
\newcommand*{\CCgt}{\sqsupset} %% opposite order on Concrete Domain
\monobioperator{\CClub}{\sqcup}{\bigsqcup}
\monobioperator{\CCglb}{\sqcap}{\bigsqcap}
\newcommand*{\CCbot}{\bot} %% bottom of Concrete Domain
\newcommand*{\CCtop}{\top} %% top of Concrete Domain

\newcommand*{\CCcpo}{\cpo{\CC}{\CCleq}}
\newcommand*{\CClattice}{\lattice{\CC}{\CCleq}{\CClub{}{}}{\CCglb{}{}}{\CCtop}{\CCbot}}

% Default Concrete Domain (for paper body, to be localized)

\newcommand*{\Clubbigsym}{\bigsqcup}
\newcommand*{\Cglbbigsym}{\bigsqcap}
\newcommand*{\Clubsym}{\sqcup}
\newcommand*{\Cglbsym}{\sqcap}

\newcommand*{\C}{\CC}
\newcommand*{\Cleq}{\CCleq}
\newcommand*{\Cnleq}{\CCnleq}
\newcommand*{\Clt}{\CClt}
\newcommand*{\Cgeq}{\CCgeq}
\newcommand*{\Cgt}{\CCgt}
\monobioperator{\Club}{\Clubsym}{\Clubbigsym}
\monobioperator{\Cglb}{\Cglbsym}{\Cglbbigsym}
\newcommand*{\Cbot}{\CCbot}
\newcommand*{\Ctop}{\CCtop}

\newcommand*{\Ccpo}{\cpo{\C}{\Cleq}}
\newcommand*{\Clattice}{\lattice{\C}{\Cleq}{\Club{}{}}{\Cglb{}{}}{\Ctop}{\Cbot}}

% Generic Abstract Domain (for preliminaries)

\renewcommand*{\AA}{\mathbb{A}}
\newcommand*{\AAleq}{\leq} %% order on Abstract Domain
\newcommand*{\AAnleq}{\nleq} %% order on Abstract Domain
\newcommand*{\AAlt}{<}
\newcommand*{\AAgeq}{\geq} %% order on Abstract Domain
\newcommand*{\AAgt}{>}
\monobioperator{\AAlub}{\vee}{\bigvee}
\monobioperator{\AAglb}{\wedge}{\bigwedge}
\newcommand*{\AAbot}{\bot} %% bottom of Abstract Domain
\newcommand*{\AAtop}{\top} %% top of Abstract Domain

\newcommand*{\AAcpo}{\cpo{\AA}{\AAleq}}
\newcommand*{\AAlattice}{\lattice{\AA}{\AAleq}{\AAlub{}{}}{\AAglb{}{}}{\AAtop}{\AAbot}}

% Default Concrete Domain (for paper body, to be localized)

\newcommand*{\Alubbigsym}[1][]{\bigvee\nolimits_{\!#1}}
\newcommand*{\Aglbbigsym}[1][]{\bigwedge\nolimits_{#1}}
\newcommand*{\Alubsym}[1][]{\vee_{#1}}
\newcommand*{\Aglbsym}[1][]{\wedge_{#1}}

\newcommand*{\A}[1][]{\AA_{#1}}
\newcommand*{\Aleq}[1][]{\AAleq_{#1}}
\newcommand*{\Anleq}[1][]{\AAnleq_{#1}}
\newcommand*{\Alt}[1][]{\AAlt_{#1}}
\newcommand*{\Ageq}[1][]{\AAgeq_{#1}}
\newcommand*{\Agt}[1][]{\AAgt_{#1}}
\monobioperatorOARG{\Alub}{\Alubsym}{\Alubbigsym}
\monobioperatorOARG{\Aglb}{\Aglbsym}{\Aglbbigsym}
\newcommand*{\Abot}[1][]{\AAbot_{#1}}
\newcommand*{\Atop}[1][]{\AAtop_{#1}}

\newcommand*{\Acpo}[1][]{\cpo{\A[#1]}{\Aleq[#1]}}
\newcommand*{\Alattice}[1][]{\lattice{\A[#1]}{\Aleq[#1]}{\Alub[#1]{}{}}{\Aglb[#1]{}{}}{\Atop[#1]}{\Abot[#1]}}

% \newcommand*{\al}{\parensmathoper{\alpha}}
% \newcommand*{\ga}{\parensmathoper{\gamma}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               %
%   Names of Standard Domains   %
%                               %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\POS}{\ensuremath{\mathcal{POS}}}

\newcommand*{\POSpreabs}[1][]{\parensmathoper{\Gamma_{#1}}}
\makeparensmathoper{\POSabs}{\alpha_{\Gamma}}
\makeparensmathoper{\POSconc}{\gamma_{\Gamma}}
\newcommand*{\POSlub}{\Alub}
\newcommand*{\POSglb}{\Aglb}
\newcommand*{\POSleq}{\Aleq}
\newcommand*{\POSrestrict}[2]{{#1}|_{#2}}
\newcommand*{\POSTp}{\Tp[g]}
\newcommand*{\POSinterp}{\I[g]}
\newcommand*{\POSeval}{\eval[g]}

\newcommand*{\Iff}{\leftrightarrow}

% still to be organized

\newcommand*{\KCTerms}[1][\KVsyms]{\SigTerms{\Csyms}{\Vsyms\cup #1}} %[1][\Fsyms]{\TermsSym(#1, )} %% terms
\newcommand*{\KI}{{\I[\kappa]}}
\newcommand*{\KSz}{\Sz[\kappa]}
\newcommand*{\KTerms}[1][\KVsyms]{\Terms[{\Vsyms\cup #1}]} %[1][\Fsyms]{\TermsSym(#1, )} %% terms
\newcommand*{\KTp}{\Tp[\kappa]}
\newcommand*{\KVsyms}{\widehat{\Vsyms}}
\newcommand*{\Kcut}[2][k]{#2 \lightning_{#1}}
\newcommand*{\Keval}{\eval[\kappa]}
\newcommand*{\depthk}[1][k]{\ensuremath{\mathit{depth}(#1)}}

% BACKWARD COMPATIBILITY

\backcompatibility{\botAA}{\AAbot}
\backcompatibility{\botA}{\Abot}
\backcompatibility{\botCC}{\CCbot}
\backcompatibility{\botC}{\Cbot}
\backcompatibility{\cpoAA}{\AAcpo}
\backcompatibility{\cpoA}{\AAcpo}
\backcompatibility{\cpoCC}{\CCcpo}
\backcompatibility{\cpoC}{\CCcpo}
\backcompatibility{\geqC}{\Cgeq}
\backcompatibility{\glbAA}{\AAglb}
\backcompatibility{\glbA}{\Aglb}
\backcompatibility{\glbCC}{\CCglb}
\backcompatibility{\glbC}{\Cglb}
\backcompatibility{\latticeAA}{\AAlattice}
\backcompatibility{\latticeA}{\Alattice}
\backcompatibility{\latticeCC}{\CClattice}
\backcompatibility{\latticeC}{\Clattice}
\backcompatibility{\leqAA}{\AAleq}
\backcompatibility{\leqA}{\Aleq}
\backcompatibility{\leqCC}{\CCleq}
\backcompatibility{\leqC}{\Cleq}
\backcompatibility{\lubAA}{\AAlub}
\backcompatibility{\lubA}{\Alub}
\backcompatibility{\lubCC}{\CClub}
\backcompatibility{\lubC}{\Club}
\backcompatibility{\nleqAA}{\AAnleq}
\backcompatibility{\nleqA}{\Anleq}
\backcompatibility{\nleqCC}{\CCnleq}
\backcompatibility{\nleqC}{\Cnleq}
\backcompatibility{\topAA}{\AAtop}
\backcompatibility{\topA}{\Atop}
\backcompatibility{\topCC}{\CCtop}
\backcompatibility{\topC}{\Ctop}


==> wgmacros-general.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                         %
%   General definitions   %
%                         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{wgmacros-absint}
\input{wgmacros-math}
\input{wgmacros-misc}
\input{wgmacros-semantics}


==> wgmacros-math.tex <==
\makeatletter
\ifx\@wgmacros@math\@relax\else\makeatother\endinput\fi
\gdef\@wgmacros@math{\relax}
\typeout{********* LOADING wgmacros-math}

\@ifpackagelater{mathtools}{2011/02/12}{%
\DeclarePairedDelimiterX{\set}[2]{\{}{\}}{#1\ifempty{#2}{}{\,\delimsize\vert\, #2}}
\DeclarePairedDelimiterX{\mset}[2]{\langle}{\rangle}{#1\ifempty{#2}{}{\,\delimsize\vert\, #2}}
}{%
\PackageWarning{WGmacros}{The version of `mathtools' package is too old, expect wrong output}
\DeclarePairedDelimiter{\set}{\{}{|}
\DeclarePairedDelimiter{\mset}{\langle}{|}
}
\makeatother

\newcommand*{\dfn}{\coloneq}
\newcommand*{\revdfn}{\eqqcolon}

\providecommand{\annote}[1]{}

\newcommand*{\cpo}[2]{{(#1, \, \mathord{#2})}}

\newcommand*{\lattice}[6]{{(#1, \, \mathord{#2}, \, \annote{$\vee$}\mathord{#3},
  \, \mathord{#4}\ifempty{#5}{}{, \,
  \annote{$\top$}\mathord{#5}, \, \mathord{#6}})}}

\newcommand*{\zseq}[2][]{\overrightarrow{{#2}_{#1}}} %% indexed (short) sequence
\newcommand*{\seq}[2][n]{#2_{1}, \dots, #2_{#1}} %% indexed sequence
\newcommand*{\hoseq}[3][n]{#2{{#3}_{1}}, \dots, #2{{#3}_{#1}}}
\newcommand*{\emptyseq}{\diamondsuit}

\newcommand*{\glb}{\ensuremath{\mathit{glb}}}
\newcommand*{\lub}{\ensuremath{\mathit{lub}}}

\newcommand*{\quotient}[2]{{#1}\big/_{\! #2}}
\newcommand*{\eqClass}[2]{[{#1}]_{#2}}

\newcommand*{\PowerSet}[1]{\mathop{\powerset}(#1)}
\newcommand*{\FinPowerSet}[1]{\mathop{\powerset_{\!\!\mathit{fin}}}(#1)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                 %
%   Macros that some package may already provide  %
%                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand*{\mathoper}[1]{\mathop{\mathit{#1}}\nolimits}

\providecommand*{\pair}[2]{{\langle #1, \, #2 \rangle}}
\providecommand*{\triple}[3]{{\langle #1, \, #2, \, #3 \rangle}}
\providecommand*{\quadruple}[4]{{\langle #1, \, #2, \, #3, \, #4 \rangle}}

\providecommand*{\true}{\mathit{true}}       %% simbolo di costante logica (T)
\providecommand*{\false}{\mathit{false}}     %% simbolo di costante logica (F)
\providecommand*{\id}[1][]{\mathit{id}_{#1}} %% funzione identica

\providecommand*{\True}{\mathit{True}}
\providecommand*{\False}{\mathit{False}}

\providecommand*{\nimplies}{\nRightarrow}
\renewcommand*{\implies}{\Rightarrow}
\providecommand*{\nimplied}{\nLeftarrow}
\providecommand*{\implied}{\Leftarrow}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                 %
%   Symbols that some package like MnSymbol may already provide   %
%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ProvideWarnCommand{\powerset}{\wp}
\ProvideWarnCommand{\llbracket}{[\![}
\ProvideWarnCommand{\rrbracket}{]\!]}

\ProvideWarnCommand{\coloneqq}{\mathrel{\vcentcolon=}} %% :=
\ProvideWarnCommand{\coloneq}{\mathrel{\coloneqq}}
\ProvideWarnCommand{\eqqcolon}{\mathrel{=\vcentcolon}} % =:

% Negated symbols
\ProvideWarnCommand{\ngg}{\not\gg}
\ProvideWarnCommand{\nin}{\notin}
\ProvideWarnCommand{\notin}{\not\in}
\ProvideWarnCommand{\npreccurlyeq}{\not\preccurlyeq}
\ProvideWarnCommand{\nsimeq}{\not\simeq}
\ProvideWarnCommand{\nsqsubseteq}{\not\sqsubseteq}
\ProvideWarnCommand{\nrightarrowtriangle}{\not\rightarrowtriangle}
\ProvideWarnCommand{\nRightarrow}{\not\Rightarrow}

% BACKWARD COMPATIBILITY

\backcompatibility{\equivClass}{\quotient}


==> wgmacros-misc.tex <==
\makeatletter
\ifx\@wgmacros@misc\@relax\else\makeatother\endinput\fi
\gdef\@wgmacros@misc{\relax}
\typeout{********* LOADING wgmacros-misc}

\@ifpackageloaded{listings}{
    \newcommand*{\mlst}[1]{\mbox{\lstinline[multicols=]`#1`}}
}{
    \newcommand*{\mlst}[1]{\fbox{\fbox{load package listings}\texttt{\string#1}}}
}

\@ifpackageloaded{datetime2}{
    \newcommand*{\currenttime}{\DTMcurrenttime}
}{
}
\makeatother

\providecommand*{\currenttime}{\fbox{NO TIME package}}
\providecommand*{\mathscr}{\PackageWarning{WGmacros}{no mathscr font}\mathcal}
\providecommand*{\mathfrak}{\PackageWarning{WGmacros}{no mathfrak font}\mathcal}

\providecommand*{\eg}   {e.g.}
\providecommand*{\etc}  {\emph{etc}.}
\providecommand*{\ie}   {i.e.,}
\providecommand*{\resp} {respectively}
\providecommand*{\st}   {s.t.}
\providecommand*{\wrt}  {w.r.t.}
\providecommand*{\wlg}  {w.l.o.g.}
% \providecommand*{\Wlog} {\wlg}
%
\newcommand*{\paradigm}[1][] {\Fbox{default #1 paradigm}}
\newcommand*{\proglang}{\Fbox{default programming language}}
\newcommand*{\program}[1][A]{\ifempty{#1}{P}{p}rogram}
\newcommand*{\programs}[1][A]{\program[#1]s}
\newcommand*{\progequiv}{\program\ equivalence}
\newcommand*{\progequivs}{\progequiv s}
\newcommand*{\progrule}{\program\ rule}
\newcommand*{\progrules}{\progrule s}
\newcommand*{\query}[1][A]{\ifempty{#1}{Q}{q}uery}
\newcommand*{\queries}[1][A]{\ifempty{#1}{Q}{q}ueries}
\newcommand*{\expression}[1][A]{\ifempty{#1}{E}{e}xpression}
\newcommand*{\expressions}[1][A]{\expression[#1]s}
\newcommand*{\deffun}[1][A]{\ifempty{#1}{defined }{}function}
\newcommand*{\deffuns}[1][A]{\deffun[#1]s}


\providecommand*{\bibURLext}[2]{\draft{CONSIDER convert bib entry with `url' field!}Available at URL: \href{#1}{\texttt{#2}}}
\providecommand*{\bibURL}[1]{\draft{CONSIDER convert bib entry with `url' field!}Available at URL: \href{#1}{\texttt{#1}}}
\providecommand*{\href}[2]{\wgmWarn{\href}\underline{#2}}

\providecommand*{\email}[1]{\texttt{#1}}

\newcommand*{\xcite}[1]{[{#1}]}

%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{color}

\definecolor{aliciacolor}{RGB}{0,125,0}

\newcommand{\Ago}[2][]{\hole{\colorbox{yellow}{Santi} #1 \quad #2}}
\newcommand{\Marco}[2][]{{\color{blue}\hole{\colorbox{yellow}{Marco} #1 \quad #2}}}
\newcommand{\MarcoPN}[2]{\begin{draftpleasenote}[Marco: #1]\color{blue} #2\end{draftpleasenote}}
\newcommand{\Maria}[2][]{\hole{\colorbox{yellow}{Maria} #1 \quad #2}}
\newcommand{\Moreno}[2][]{\hole{\colorbox{yellow}{Moreno} #1 \quad #2}}

\newcommand{\Alicia}[2][]{\hole{\textbf{#1}\hfill{\color{aliciacolor}\textbf{Alicia}}\\[-1.7ex]\rule{\linewidth}{0.5mm}\\ #2}}
\newcommand{\Giovanni}[2][]{\hole{\textbf{#1}\hfill{\color{blue}\textbf{Giovanni}}\\[-1.7ex]\rule{\linewidth}{0.5mm}\\ #2}}

% nonstandard color names

\RequirePackage{xcolor}

\newcommand{\FromTo}[2]{\csname#1\endcsname[\colorbox{pink}{@#2}]}

\newcommand{\Laura}[2][]{\hole{\textbf{#1}\hfill{\color{violet}\textbf{Laura}}\\[-1.7ex]\rule{\linewidth}{0.5mm}\\ #2}}
\newcommand{\Luca}[2][]{\hole{\textbf{#1}\hfill{\color{orange}\textbf{Luca}}\\[-1.7ex]\rule{\linewidth}{0.5mm}\\ #2}}
\newcommand{\MarcoA}[2][]{\hole{\textbf{#1}\hfill{\color{orange}\textbf{MarcoA}}\\[-1.7ex]\rule{\linewidth}{0.5mm}\\ #2}}

% \newcommand{\AtAlicia}{\FromTo{Marco}{Alicia}}%[1]\Marco[\colorbox{pink}{@Alicia}]{#1}}
% \newcommand{\AtGiovanni}{\FromTo{Marco}{Giovanni}}%[1]{\Marco[\colorbox{pink}{@Giovanni}]{#1}}
% \newcommand{\AtLaura}{\FromTo{Marco}{Laura}}%[1]{\Marco[\colorbox{pink}{@Laura}]{#1}}
% \newcommand{\AtLuca}{\FromTo{Marco}{Luca}}%[1]{\Marco[\colorbox{pink}{@Luca}]{#1}}



==> wgmacros-semantics.tex <==
\makeatletter
\ifx\@wgmacros@semantics\@relax\else\makeatother\endinput\fi
\gdef\@wgmacros@semantics{\relax}
\typeout{********* LOADING wgmacros-semantics}

\providecommand{\ifempty}[3]{\def\@@@temp{#1}\ifx\@@@temp\@empty#2\else#3\fi}
\@ifpackageloaded{mathtools}{}{\PackageWarning{WGmacros}%
{Please load `mathtools' package explicitely in preamble}
\makeatother
\RequirePackage{mathtools}}

\input{wgmacros-support}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%                        %
%   DOMAINS and orders   %
%                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\Cinterps}[1][\C]{\mathbb{I}_{#1}} %% interpretations
\newcommand*{\Ainterps}[1][\A]{\mathbb{I}_{#1}} %% interpretations
\newcommand*{\CIleq}{\Cleq} %% order on interpretetions
\newcommand*{\AIleq}{\Aleq} %% order on interpretetions
\newcommand*{\CInleq}{\Cnleq} %% order on interpretetions
\newcommand*{\AInleq}{\Anleq} %% order on interpretetions

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       %
%   TERMS (signature, positions, ...)   %
%                                       %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% private (just for redefinition)
\newcommand*{\mathT}{\mathcal}
\newcommand*{\TermsSym}{\mathT{T}}
\newcommand*{\LinTermsSym}{\mathT{L}{\scriptstyle\TermsSym}}
\newcommand*{\twoParsDenot}[3]{\mathop{#1}(#2\ifempty{#3}{}{,#3})}
% public

\newcommand*{\SigTerms}[2]{\twoParsDenot{\TermsSym}{#1}{#2}}
\newcommand*{\LinSigTerms}[2]{\twoParsDenot{\LinTermsSym}{#1}{#2}}

\newcommand*{\Psyms}{\Pi}       %% predicate symbols (signature)
\newcommand*{\Fsyms}{\Sigma}    %% function symbols (signature)
\newcommand*{\Csyms}{\mathT{C}} %% constructor symbols
\newcommand*{\Dsyms}{\mathT{D}} %% defined symbols
\newcommand*{\Vsyms}{\mathT{V}} %% variable symbols
\backcompatibility{\Fsym}{\Fsyms}
\backcompatibility{\Csym}{\Csyms}
\backcompatibility{\Dsym}{\Dsyms}
\backcompatibility{\Vsym}{\Vsyms}

\newcommand*{\unravel}[1]{\lbag #1 \rbag}



%% terms
\newcommand*{\Terms}[1][\Vsyms]{\SigTerms{\Fsyms}{#1}}
\newcommand*{\CTerms}[1][\Vsyms]{\SigTerms{\Csyms}{#1}}
\newcommand*{\LinTerms}[1][\Vsyms]{\LinSigTerms{\Fsyms}{#1}}
\newcommand*{\LinCTerms}[1][\Vsyms]{\LinSigTerms{\Csyms}{#1}}
\newcommand*{\TreeTerms}[1][\Vsyms]{\twoParsDenot{\mathbb{T}}{\Csyms}{#1}}

\newcommand*{\leqT}{\preceq} %% order on terms

% \newcommand*{\leqP}{\fbox{change}\preceq} %% order on positions
% \newcommand*{\pos}[2][]{\mathcal{O}_{#1}(#2)} %% term positions set
\newcommand*{\append}{\cdot} %% append
\newcommand*{\replace}[3]{#1[#2]_{#3}} %% term replacement
\newcommand*{\rootPos}{\Lambda} %% root position
\newcommand*{\subterm}[2]{#1|_{#2}} %% subterm

\makeparensmathoper{\vars}{var} %% term variables
\newcommand*{\fresh}{\ll} %% fresh variant

\newcommand*{\termres}[2]{{#1} \ifempty{#2}{}{\triangleright {#2}}}

\newcommand*{\call}[3]{\termres{\mathit{#1}\ifempty{#2}{}{\mathit{(#2)}}}{#3}}
\newcommand*{\mgc}[4][]{\call{#2}{{\zseq[#1]{#3}}}{#4}}

%% program (rewrite) rule
\newcommand*{\genrule}[2]{#1 \rightarrow #2}
\newcommand*{\prule}[3]{\genrule{\mathit{#1}\ifempty{#2}{}{\mathit{(#2)}}}{#3}}

\newcommand*{\mghead}[3][]{\mathit{#2}\ifempty{#3}{}{(\zseq[#1]{\mathit{#3}})}}
\newcommand*{\mgrule}[4][]{\genrule{\mghead[#1]{#2}{#3}}{#4}}

% \newcommand*{\letop}[2]{\mathop{\mathit{let}} #1 \mathrel{\mathit{in}} #2 } %% let constr. (abstract syntax)

%%%%%%%%%%%%%%%%%%%%%
%                   %
%   SUBSTITUTIONS   %
%                   %
%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\Substs}{\mathit{Substs}}
\newcommand*{\CLinSubsts}{\Csyms\mathit{lin}\Substs}
\newcommand*{\CSubsts}{\Csyms\Substs} %% constructor substitutions
\newcommand*{\MGCsym}{\mathbb{MGC}}
\newcommand*{\MGC}[1][]{\MGCsym_{#1}} %% most general call set

\newcommand*{\leqS}{\preceq} %% order on substitutions
\newcommand*{\gtS}{\succ}    %% order on substitutions
\newcommand*{\eqS}{\simeq}    %% order on substitutions
\newcommand*{\neqS}{\nsimeq}    %% order on substitutions
% \newcommand*{\lubS}{\mathbin{\uparrow}} % oppure mathrel?
\monobioperator{\lubS}{\mathbin{\uparrow}}{\mathbin{\uparrow}}

\newcommand*{\emptysubst}{\varepsilon} %% empty substitution
\makeparensmathoper{\dom}{dom} %% domain
\makeparensmathoper{\range}{range} %% range
\makeparensmathoper{\img}{img}
\backcompatibility{\domrestriction}{\restrict}
\newcommand*{\restrict}[2]{{#1}\mathord{\restriction}_{#2}} %% domain restriction
\newcommand*{\restrictVars}[2]{\restrict{#1}{\vars{#2}}}

%%%%%%%%%%%%%%%%
%              %
%   PROGRAMS   %
%              %
%%%%%%%%%%%%%%%%

\newcommand*{\ProgsSym}{\mathbb{P}}
\newcommand*{\Progs}[1][\Fsyms]{\ProgsSym_{#1}} % \mathit{Progs}

\newcommand*{\ProgSym}{P}
\newcommand*{\prog}[1][]{\ensuremath{\ProgSym_{\mathit{#1}}^{}}} %% generic program
\renewcommand*{\P}{\prog} %% generic program Alias

\newcommand*{\CAnsw}[2]{{#1 \cdot #2}}%\talloblong\mathrel{}
\backcompatibility{\cansw}{\CAnsw}
\newcommand*{\CAleq}{\preceq}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                             %
%   REWRITING AND NARROWING   %
%                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \RequirePackage{theorems}
\providecommand*{\starred}[2][*] {\wgmWarn{\starred}\mathrel{\mathord{#2}{}^{#1}}}


\newcommand*{\rewriteStep}[2][\genrule{l}{r}]{\xrightarrow[{#1}]{#2}}
% \newcommand*{\rewriteStep}[2][\genrule{l}{r}]{\xrightarrow[{\scriptscriptstyle #1}]{\scriptscriptstyle #2}}
\newcommand*{\rewrites}[1][]{\rewriteStep[{#1}]{}}
\newcommand*{\rewritesTo}[1][]{\starred{\rewrites[{#1}]}}
\newcommand*{\nrewrites}{\nrightarrow}
\newcommand*{\nrewritesTo}{\starred{\nrewrites}}


\newcommand*{\narrows}[2][]{\mathrel{\mathop{\leadsto}\limits^{\scriptscriptstyle #2}_{\scriptscriptstyle #1}}}
\newcommand*{\narrowsTo}[2][]{\starred{\narrows[#1]{#2}}}
\newcommand*{\narrowStep}[3][\genrule{l}{r}]{\narrows[{#1}]{\extraArg{#2}{#3}}}
\newcommand*{\nnarrows}{\not\leadsto}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        %
%   SEMANTICS INTERPRETATION FUNCTIONS   %
%                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% private (just for redefinition)
\newcommand*{\mathC}{\mathcal}
\newcommand*{\BehaSym}{\mathC{B}}
\newcommand*{\SemSym}{\mathC{S}}
\newcommand*{\TrSym}{\mathC{N}}
\newcommand*{\OsemSym}{\mathC{O}}
\newcommand*{\FSym}{\mathC{F}}
\newcommand*{\TpSym}{\mathC{P}}
\newcommand*{\evalSym}{\mathC{E}}
% public

\newcommand*{\Q}[2]{#1 \mathbin{\scriptstyle\mathit{in}} #2} % _ in _
\newcommand*{\Beha}[2][ss]{\syntaxoper{\BehaSym^{\mathit{#1}}}{#2}{}} %% general behavior macro
\newcommand*{\Sem}[2][\alpha]{\syntaxoper{\SemSym^{#1}}{#2}{}} % a semantics S
\newcommand*{\Tr}[3][]{\syntaxoperEXT{#2}{\TrSym_{#1}}{\Q{#2}{#3}}{}} %% semantics tree in P
% \newcommand*{\CA}[1]{\syntaxoper{\mathcal{CA}}{#1}{}} %% computed answers
% \newcommand*{\CAin}[2]{\CA{\Q{#1}{#2}}} %% computed answers in P

\newcommand*{\Osem}[1]{\syntaxoper{\OsemSym}{#1}{}} %% oper lfp characterization
\newcommand*{\F}[2][\alpha]{\syntaxoper{\FSym^{#1}}{#2}{}} %% general lfp macro
\newcommand*{\Tp}[3][\alpha]{\syntaxoper{\TpSym^{#1}}{#2}{{#3}}} %% general fixed-point op macro
\newcommand*{\TpN}[3][\alpha]{\iter{\Tp[{#1}]{#2}{}}{#3}} %% n-th iteration of the lfp conctruction
\newcommand*{\eval}[4][\alpha]{\syntaxoperEXT{#3}{\evalSym^{#1}}{\termres{#3}{#2}}{#4}}
\newcommand*{\evalrules}[3][\alpha]{\syntaxoper{\xi^{#1}}{#2}{#3}}
\newcommand*{\FUNeq}{\cong} %% variance on trees

\newcommand*{\I}[1][\alpha]{\Isym{#1}} %% generic interpretation
\newcommand*{\Sz}[1][\alpha]{\Ssym{#1}} %% generic specification
\newcommand*{\Rz}[1][\alpha]{\Rsym{#1}}
\newcommand*{\Isym}[1]{\mathC{I}^{#1}}
\newcommand*{\Ssym}[1]{\mathC{S}^{#1}}
\newcommand*{\Rsym}[1]{\mathC{X}^{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                          %
%   PROGRAM EQUIVALENCES   %
%                          %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\ProgEquiv}[3][]{#2 \thickapprox_{#1} #3} % program equivalence
\newcommand*{\nProgEquiv}[3][]{#2 \not\thickapprox_{#1} #3} % negated program equivalence
\newcommand*{\BehaEq}[1][ss]{\ProgEquiv[\mathit{#1}]}
\newcommand*{\SemEq}[1][{\F[]{}}]{\ProgEquiv[{#1}]} %% program small-step operational equivalence


%%%%%%%%%%%%%%%%%%%
%                 %
%   PROOF TREES   %
%                 %
%%%%%%%%%%%%%%%%%%%

\newcommand{\ands}{\fbox{this should not be used, is just to prevent
    unobserved redefinition of command \string\ands}}
\newcommand*{\sequent}[4][]{\gdef\and{\quad\hfill}
    \gdef\ands{\;\hfill\ldots\hfill\;}\global\setlabel{#1}
    {#1}\frac{\:\:#2\:\:}{\;#3\;}\;\text{\small%
\begin{tabular}{@{}l@{}} #4 \end{tabular}}}

\newcommand*{\twsequent}[3][]{\Fbox{OBSOLETE}\sequent[{#1}]{#2 \and #3}}

\newcommand*{\thsequent}[4][]{\Fbox{OBSOLETE}\sequent[{#1}]{#2 \and #3 \and #4}}

\newcommand*{\manysequent}[3][]{\Fbox{OBSOLETE}\sequent[{#1}]{#2 \ands #3}}

%%%%%%%%%%%%%
%           %
%   TREES   %
%           %
%%%%%%%%%%%%%

\DeclarePairedDelimiter{\Theight}{|}{|}
% \newcommand*{\Tleaf}{\parensmathoper{leaf}} %% leaf nodes of a tree
% \newcommand*{\Tsteps}{\parensmathoper{steps}} %% steps set of a tree
% \newcommand*{\Tstep}[4]{\quadruple{#1}{#2}{#3}{#4}} %% a relaxed-step in a tree
% \newcommand*{\Tsubterm}[2]{\left. #1 \right\Downarrow_{#2}} %% induced subterm tree
\newcommand*{\Tnode}[2]{\CAnsw{#1}{#2}} %% node constructor
\makeparensmathoper{\Tedges}{edges}
\makeparensmathoper{\Tleaves}{leaves} %% leaf nodes of a tree
\makeparensmathoper{\Tmaxpaths}{maxpaths}
\makeparensmathoper{\Tnodes}{nodes}
\makeparensmathoper{\Tpaths}{paths}
\makeparensmathoper{\Troot}{rt} %% root node of a tree
\makeparensmathoper{\Tsiblings}{siblings}
\makeparensmathoper{\Tsons}{sons}


%%%%%%%%%%%%%%%%%%%%%
%                   %
%   Miscellaneous   %
%                   %
%%%%%%%%%%%%%%%%%%%%%

\makeparensmathoper{\mgu}{mgu} %% most general unifier

\newcommand*{\lfp}[1][]{\lfpof[{#1}]{}}
\newcommand*{\gfp}[1][]{\gfpof[{#1}]{}}
\newcommand*{\lfpof}[2][]{\mathoper{lfp}_{#1}\Braces{#2}}
\newcommand*{\gfpof}[2][]{\mathoper{gfp}_{#1}\Braces{#2}}

\newcommand*{\downiter}[2]{#1 \mathord{\downarrow} #2} %% iteration macro
\newcommand*{\iter}[2]{#1 \mathord{\uparrow} #2} %% iteration macro
\newcommand*{\sameof}[3]{#1 \mapsto \iter{#2}{#3} (\mathit{#1})}


\makeparensmathoper{\len}{length}
\makeparensmathoper{\prefixtree}{prfxtree}


% BACKWARD COMPATIBILITY

\backcompatibility{\CSubst}{\CSubsts}
\backcompatibility{\Subst}{\Substs}
\backcompatibility{\Symbols}{\Fsyms}
\backcompatibility{\emptypos}{\rootPos}
\backcompatibility{\interpA}{\Ainterps}
\backcompatibility{\interpC}{\Cinterps}
\backcompatibility{\interp}{\Cinterps}

\backcompatibility{\leqIa}{\AIleq}
\backcompatibility{\leqIc}{\CIleq}
\backcompatibility{\leqI}{\CIleq}
\backcompatibility{\nleqIa}{\AInleq}
\backcompatibility{\nleqIc}{\CInleq}
\backcompatibility{\nleqI}{\CInleq}
\backcompatibility{\nrew}{\nrewrites}
\backcompatibility{\rewrule}{\genrule}
\newcommand*{\rews}[2][noOpt]{\Fbox{USE \texttt{\string\rewritesTo}}\Fbox{$#1$}\rewritesTo[{#2}]}
\newcommand*{\rew}[2][noOpt]{\Fbox{USE \texttt{\string\rewrites}}\Fbox{$#1$}\rewrites[{#2}]}


==> wgmacros-support.tex <==
\makeatletter
\ifx\@wgmacros@support\@relax\else\makeatother\endinput\fi
\gdef\@wgmacros@support{\relax}
% \typeout{********* LOADING wgmacros-support}
\makeatother

\RequirePackage{color}
\RequirePackage{xcolor}

\providecommand*{\Fbox}{\fcolorbox{black}{yellow}}
\providecommand*{\Flbox}{\fcolorbox{black}{lightyellow}}
\providecommand*{\Dbox}[1]{\draft{\Fbox{#1}}}

% internals

\providecommand*{\wgmWarn}[1]{\typeout{*** using WgMacros def of \string#1}}
\providecommand*{\ProvideWarnCommand}[2]{\providecommand*{#1}{\wgmWarn{#1}#2}}

\providecommand*{\backcompatibility}[2]{
  \newcommand*{#1}{\Fbox{USE \texttt{\string#2}}#2}
}
\providecommand*{\warnUpgrade}[2]{\typeout{****** WgMacros warning: use \string#1\{..\}\{\string#2\}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                      %
%   Support (General Purpose) Macros   %
%                                      %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand*{\makeparensmathoper}[2]{
  \newcommand*{#1}[2][]{\ensuremath{\mathoper{#2}\ifempty{##2}{}{##1(##2##1)}}}
}
\providecommand*{\makeparensmathoperEXT}[2]{
  \newcommand*{#1}[2][]{\ensuremath{\mathoper{#2}\ifempty{##2}{}{##1(##2##1)}}}
}

\providecommand*{\monobioperator}[3]{
  \newcommand*{#1}[2]{{\ifempty{##2}{#3##1}{##1#2##2}}}
}
\providecommand*{\monobioperatorOARG}[3]{
  \newcommand*{#1}[3][]{{\ifempty{##3}{#3[##1]##2}{##2#2[##1]##3}}}
}

\providecommand*{\parensmathoper}[3][]{\warnUpgrade{\makeparensmathoper}{#2}\ensuremath{\mathoper{#2}\ifempty{#3}{}{#1(#3#1)}}}
\providecommand*{\parensmathoperEXT}[4][]{\warnUpgrade{\makeparensmathoperEXT}{#2}\ensuremath{\mathoper{#2}\ifempty{#3}{}{#1(#4#1)}}}
\providecommand*{\syntaxoper}[3]{\mathoper{#1}\BBrackets[#3]{#2}}
\providecommand*{\syntaxoperEXT}[4]{\mathoper{#2}\ifempty{#1}{}{\llbracket#3\rrbracket_{#4}}}%

\providecommand*{\BBrackets}[2][]{\ifempty{#2}{}{\llbracket#2\rrbracket_{#1}}}
\providecommand*{\Braces}[2][]{\ifempty{#2}{}{( #2 )_{#1}}}%\big\big
\providecommand*{\extraArg}[2]{\ifempty{#1}{#2}{\ifempty{#2}{#1}{#1 ,\, #2}}}
\providecommand*{\extraArgSc}[2]{\ifempty{#2}{#1}{\ifempty{#1}{#2}{#1 ;\, #2}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                            %
%   Support Macros defined by theorems.sty   %
%                                            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand*{\newsmartprefix}[2]{\wgmWarn{\newsmartprefix}}
\providecommand*{\newsmartsprefix}[2]{\wgmWarn{\newsmartsprefix}}
\providecommand*{\newdefinition}[1]{\wgmWarn{\newdefinition}\newdefinitionaux}
\providecommand*{\newdefinitionaux}[2][]{}
